Comparing models of the periodic variations in spin-down and beam-width for PSR B1828-11

We build a framework using tools from Bayesian data analysis to evaluate models explaining the periodic variations in spin-down and beam-width of PSR B1828-11. The available data consists of the time averaged spin-down rate, which displays a distinctive double-peaked modulation, and measurements of the beam-width. Two concepts exist in the literature that are capable of explaining these variations; we formulate predictive models from these and quantitatively compare them. The first concept is phenomenological and stipulates that the magnetosphere undergoes periodic switching between two meta-stable states as first suggested by Lyne et al. The second concept, precession, was first considered as a candidate for the modulation of B1828-11 by Stairs et al.. We quantitatively compare models built from these concepts using a Bayesian odds-ratio. Because the phenomenological switching model itself was informed by this data in the first place, it is difficult to specify appropriate parameter-space priors that can be trusted for an unbiased model comparison. Therefore we first perform a parameter estimation using the spin-down data, and then use the resulting posterior distributions as priors for model comparison on the beam-width data. We find that a precession model with a simple circular Gaussian beam geometry fails to appropriately describe the data, while allowing for a more general beam geometry provides a good fit to the data. The resulting odds between the precession model (with a general beam geometry) and the switching model are estimated as $10^{2.7 \pm 0.5}$ in favour of the precession model.

==> Table_Beamwidth_ModifiedGaussian_posterior.tex <==
\begin{tabular}{lll} \hhline{===}
        Parameter & Mean $\pm$ s.d. &  Units\\ \hline
$\tau_{P}$ & $485.0$$\pm$0.4685 & days\\
$P$\textrm{-}$P^{\tiny\textrm{ATNF}}$
 & ${\text{\textrm{-}}3.76}\times 10^{\textrm{-}14}$$\pm$${1.19}\times 10^{\textrm{-}11}$ & s\\
$\theta$ & 0.049$\pm$0.002 & rad\\
$\chi$ & 1.552$\pm$0.001 & rad\\
$\psi_0$ & 3.970$\pm$0.040 & rad\\
$\rho_{2}^{0}$ & 0.025$\pm$0.000 & rad\\
$\rho_{2}''$ & 3.4414$\pm$0.3887 & rad$^{\textrm{-}2}$\\
$\cos(\iota)$ & ${7.92}\times 10^{\textrm{-}3}$$\pm$${1.92}\times 10^{\textrm{-}3}$ & \\
$\sigma_{W_{10}}$ & 1.5834$\pm$0.0423 & ms\\
\hhline{===}
\end{tabular}

==> Table_Beamwidth_ModifiedGaussian_prior.tex <==
\begin{tabular}{lll} \hhline{===}
        Parameter & Distribution &  Units\\ \hline
$\tau_{P}$$^{*}$ & $\mathcal{N}$($485.6$, 0.8188) & days\\
$P$\textrm{-}$P^{\tiny\textrm{ATNF}}$
$^{*}$ & $\mathcal{N}$(${1.04}\times 10^{\textrm{-}14}$, ${1.19}\times 10^{\textrm{-}11}$) & s\\
$\theta$$^{*}$ & $\mathcal{N}$(0.049, 0.002) & rad\\
$\chi$$^{*}$ & $\mathcal{N}$(1.552, 0.001) & rad\\
$\psi_0$$^{*}$ & $\mathcal{N}$(3.871, 0.070) & rad\\
$\rho_{2}^{0}$$^{}$ & Unif(0, 0.150) & rad\\
$\rho_{2}''$$^{}$ & $\mathcal{N}$(0, 7) & rad$^{\textrm{-}2}$\\
$\cos(\iota)$$^{}$ & Unif(\textrm{-}1, 1) & \\
$\sigma_{W_{10}}$$^{}$ & Unif(0, 5) & ms\\
\hhline{===}
\end{tabular}
